A Top-Down Approach to Managing Variability in Robotics Algorithms

One of the defining features of the field of robotics is its breadth and heterogeneity. Unfortunately, despite the availability of several robotics middleware services, robotics software still fails to smoothly handle at least two kinds of variability: algorithmic variability and lower-level variability. The consequence is that implementations of algorithms are hard to understand and impacted by changes to lower-level details such as the choice or configuration of sensors or actuators. Moreover, when several algorithms or algorithmic variants are available it is difficult to compare and combine them. In order to alleviate these problems we propose a top-down approach to express and implement robotics algorithms and families of algorithms so that they are both less dependent on lower-level details and easier to understand and combine. This approach goes top-down from the algorithms and shields them from lower-level details by introducing very high level abstractions atop the intermediate abstractions of robotics middleware. This approach is illustrated on 7 variants of the Bug family that were implemented using both laser and infra-red sensors.

==> section2.tex <==
\section{Case study: Bug algorithms}
In this section, we illustrate our approach on the Bug family of navigation algorithms. It is symptomatic that even with a very simplified assumptions underlying a family of algorithms it is still difficult
\begin{itemize}
\item to understand the differences among the algorithmic variants,
\item to choose one variant over another,
\item to share development efforts among variants.
\end{itemize} 

\subsection{Bug algorithms overview}
The Bug algorithms attempt solve the navigation problem in an unknown two-dimensional environment with fixed obstacles and a known goal position. Over 20 versions of Bug algorithms have been defined in the literature. Among them, 7 variants are considered in this paper.

The Bug algorithms share the following assumptions~\cite{Lumelsky84} : 1) The environment is unknown and a finite number of fixed obstacles are placed arbitrarily.
2) The robot is considered as a point (i.e it has no body). It has perfect sensors (for obstacles detection) and a perfect localization ability (e.g. to compute its distance to its goal).

The inputs of the Bug algorithms are the robot's start position and the target position. At the end of the algorithm's execution, the robot must indicate if its goal is reached or 
if the goal is unreachable. Most of the Bug algorithms can be programmed on any mobile robot using tactile or distance sensing  and a localization method while some require distance sensing.



\subsection{Abstractions identification}
%\subsubsection{Rational}
%Qu'est-ce que l'on fait : prendre des algorithmes existants (et leurs variantes) qui sont sous forme de pseudo-code, de code, de descriptions textuelles + identifier la famille de capteurs nécessaires à ces algorithmes. Identifier des "abstractions" et leurs enchainements (comportements, conditions d'activations, types de données (?)) communs à l'ensemble des algorithmes.
%
%Pourquoi on le fait: arriver à une description générique de l'algorithme
%Starting from existing algorithms descriptions (textual descriptions, pseudo-code) and from the requisite sensors to define them, we can identify appropriate abstractions, the variant parts of the algorithms which must be specified in terms of these abstractions and the invariant parts among all algorithms (behaviors, activation conditions, data types). The usefulness of this approach is to extract a specification of a generic hardware-independent algorithm.

%\subsubsection{Application to Bug Algorithm Family}
%%Les Bug Algorithms sont organisés de la même façon qu'un algorithmique robotique (décomposition en Sense-Plan-Act).
%%Notre approche pourra donc être utilisé dans d'autres contextes.
%Let us illustrate this step on our example. Bug algorithms are organised with respect to any robotics algorithm architecture: Sense-Plan-Act. Hence, our approach could be applied to other robotics applications. 

In the litterature, as far as we know, Bug algorithms are only published with an informal description.
Bug algorithms are very similar fundamentally but differ in some points of interest. Their principle is the following: (1) The robot motion to its goal until an obstacle is detected on its way. (2) 
The robot looks then for a point (called leave point) around the encountered obstacle to be able to move to its goal again from this point. (3) When a leave point is identified, the robot moves 
to it and leaves the obstacle. 
Steps (1), (2) and (3) are repeated until the robot reaches its goal or until the robot indicates that the goal is unreachable.
This description of Bug gathers hardware variability which impacts on obstacle detection and localisation tasks and algorithmic variability which is related to the leave point identification task.
In this section, we aim to define the appropriate abstractions for Bug family algorithms.

\paragraph{Behaviors}

Following a goal directed approach
%The default behavior of the robot when there is no obstacle encountered on its way to the goal is \texttt{motion to goal}. This behavior consists in moving in a straight line to the goal from the robot's current position.\\
%When an \emph{obstacle is detected}, the robot checks whether the goal is reached by calculating the euclidian distance from its \emph{current position} to the goal. If the goal \texttt{is reached}, the algorithm returns success and the robot stops. Otherwise, the robot switches from motion to goal to obstacle avoidance mode to \texttt{try to leave} the encountered obstacle and to motion to the goal again.\\
%While switching from motion to goal to obstacle avoidance, the robot \texttt{records several data} depending on the algorithm. For instance, in almost all studied Bug algorithms here, the robot records the hit point. However, in Tangent Bug, in addition to recording the hit point, the robot computes discontinuity points~\cite{Kamon98}, heuristic distance and the \emph{rotation angle} and go to the point which minimizes its heuristic distance to the goal.\\
%In all the algorithms, after recording data and the computation step (only for TangentBug), the robot starts following the boundary of the encountered obstacle (behavior \texttt{boundary following}) in a specific \textit{direction} while looking for a leave point (a point which satisfies the algorithm specific strategy and from which the robot can motion to its goal again). \\
%If the leave point is identified, the robot goes to that point and switches to motion to goal again. In almost all the algorithms that we have studied, if the robot does not find a leave point until it performs a \texttt{complete cycle around the encountered obstacle}, the algorithm returns failure and the robot stops except for the algorithm Bug1~\cite{Lumelsky84} where the leave point is identified while performing a complete cycle around the encountered obstacle. If the goal is unreachable after returning to the leave point, the algorithm returns failure. Otherwise, if the \texttt{goal is reachable} from the leave point (no visible obstacle from the leave point and the goal), the robot switches again to the behavior \texttt{motion to goal} after applying the algorithm \texttt{specific leaving treatment} (e.g: recording the leave point).

%\paragraph{Activation conditions of behaviors}
%These conditions aim at activating the behaviors presented previously. \emph{ObstacleInWay} activates the behavior obstacle avoidance. Variability in this condition is related to the used sensors type (distance or tactile).
%\emph{Leaving the obstacle avoidance} behavior represents an important variation point among Bug algorithms. We distinguish similar leaving conditions among algorithms from specific leaving conditions to algorithms. The conditions \textit{complete Cycle Around Obstacle} and \textit{goal Reachable} are checked in all Bug algorithms while some of the leaving conditions are tested only in some variants of Bug algorithms. For instance, the \textit{encountered points condition}, used in Alg1~\cite{Noborio00} and Alg2~\cite{Sankaranarayanar90:Alg2}, is defined to overcome the situations where the robot can find itself in an overlasting loop around obstacles or to find a shorter path to the goal. Regarding the specific leaving conditions, they differ from one algorithm to another:
%\begin{itemize}
%\item \textbf{The closest point around obstacle boundary condition.} It consists on recording the closest point to the goal among all the points ever visited by the robot while performing boundary following\cite{Lumelsky84, Lumelsky86}.
%\item \textbf{The m-line detection condition.} It is a straight line between the starting point and the target which aims at providing a set of prededefined leave points. The robot must leave only on these points\cite{Lumelsky86}\cite{Noborio00}.
%\item \textbf{The local minimum condition.} Using its distance sensors, the robot can detect discontinuity points\cite{Kamon98} on obstacles on its way with respect to the target.
%\item \textbf{The disabling segment condition.} A disabling segment occurs when the robot cannot move to its goal from all points in a segment while perfoming boundary following.
%\item \textbf{The step method.} The robot uses its distance sensors to detect a point which is \textit{STEP}\cite{Kamon95} closer to the target than any point already visited.
%\end{itemize}

%Two termination states could be implied by the conditions presented above, goalReached (success) and goalUnreachable (failure: when the robot knows that it cannot achieve its goal).


==> section31.tex <==
\section{Variability management}

Chapeau à écrire ici ...

\subsection{Template Method design pattern}
\subsubsection{Description}
The Template Method design pattern~\cite{Gamma95} defines an algorithm skeleton in an abstract class as a template method. This method defines the basic step of the algorithm as "placeholders" methods (or hook methods), that are different in each subclasses. Invariants parts of the algorithm are represented once in the abstract class as concrete methods. Abstract methods will be used to represent needed operations that are different in each subclasses. The main idea is to represent the variants of the algorithm as subclasses that implement these "placeholders" methods.

La configuration se fait en choisisant une sous-classe de Bug.

Variabilité des senseurs = ne pas utiliser de sous-classes (explosion combinatoire),
plutôt une délégation correspondant aux capteurs.

Une hiérarchie pour le contrôle, une hiérarchie pour chaque capteurs, une hiérarchie pour chaque actuateurs. Query = interface (au sens de Java), virtual sensors = Adateurs = classe concrète

Démarche qui peut être appliquée récursivement pour chaque composant.

\subsubsection{Application}
In this section, we apply the TM pattern to the Bug Algorithms family where every variants will be represented as specific subclasses.

\begin{tiny}
\begin{algorithm}%[H]
\hspace{-1cm}
\label{try-to-leave}
\caption{try to leave method}
%Input Data
\SetKwData{target}{$q_{goal}$}
%Variables
\SetKwData{minDistGoal}{$minDist2Goal$}
\SetKwData{total}{$totalPathLength$}
\SetKwData{pathToMin}{$length2lPoint$}
\SetKwData{traveled}{$pathTraveled$}
%leavePoint
\SetKwData{leavePoint}{$q_L^i$}
%localisation
\SetKwFunction{loc}{getRobotPosition()}
%compare euclidian distance between a point and the goal and the current position and the goal
%basic actions
\SetKwFunction{wall}{wallFollowing}

  \begin{algorithmic}
   %\Require{$dir$ is already specified}
    \Function{tryToLeave}{$Boolean \ termination$}{\\
      \BlankLine
 	bool cond = false\;
	\If{specificLeavingCondition()}{
		\If{goalIsReachable()}{
			specificLeavingTreatment()\;
			 cond = true\;
		}
	}
	\ElseIf{completeCycleAroundObstacle (getLatestHitPoint(), \loc)}{
		completeCycleAroundObstacleTreatment()\;
		cond = true\;
	}
	\ElseIf{encounteredPointsCondition (\loc)}{
		encounteredPointsTreatment()\;
	}
	\ElseIf{goalReached()}{
		termination = true\;
		cond = true\;
	}
	return cond\;
 }
 \textbf{end}
\EndFunction
   \end{algorithmic}
\end{algorithm}
\end{tiny}
As we have shown in the previous section, Bug algorithms follow the same basic schema but differ in numerous ways (recording or not environment data, 
different leaving conditions). Let us consider an abstract class \texttt{BugAlgorithm} which contains a Template Method and the following concrete, abstract and hook operations:

\begin{itemize}
\item Initialisation method (\textit{init()}) that differs in every algorithms is defined as abstract.
\item Basic robot behaviors (i.e: \textit{stop()}, \textit{wallFollowing()} and \textit{motionToGoal()}) should be normally be defined as asbtract methods but as we did'nt care at the moment about actuactors variability, we prefer to define them as concrete.
\item Perception (\textit{obstacleInWay()}) and localization methods (\textit{getRobotPosition()}) used in all algorithms are defined as abtract operations. Sensors variability is introduced as specific subclasses for each sensors.
\item Depending on the algorithms, the robot records either the last point of blocking (hit point) or all the points where it encountered several obstacles, except for Tangent Bug where additional information are recorded.
We define \textit{setHitPoint(Point)} as an abstract method which will be specialized in subclasses depending on if the robot must remember all the encountered points or not.

We also define a hook operation \textit{discontinuityPointsTreatment()} with a default empty behavior and which will be defined in the subclass corresponding to TangentBug to compute the discontinuity points and other data and go to the point with a minimum heuristic distance. (???)

\item Boundary following (which calls the simple motion \textit{wallFollowing()}) is defined as a concrete operation with one parameter: $direction$.

Regarding updated data during boundary following, they differ from one algorithm to another. Consequently, a hook method \textit{updateData()} is defined with an empty body by default (see algorithm \ref{BF-generic}). The recorded data are declared as attributes of the concrete class where they are used. For instance, in Tangent Bug, a new attribute $distFollowed$ is declared.
\item tryToLeave() is a concrete operation which calls all the leaving conditions (see algorithm \ref{try-to-leave}). Each leaving condition consists of concrete, primitive and hook operations:
\begin{itemize}
\item Complete-cycle-around-obstacle is defined as a concrete operation.
\item Encountered-Points-Condition is defined as a hook operation with an empty body by default which will be extended by the concerned algorithms (in particular, Alg1 and Alg2).
\item Specific-Leaving-Condition is defined as a primitive operation that subclasses will define.
\item Goal-Reachability-Condition is defined as a concrete operation.
\end{itemize}
\end{itemize}
The resulting algorithm is presented in the algorithm \ref{AlgGen}.
\begin{small}
\begin{algorithm}%[H]
\label{BF-generic}
\caption{BoundaryFollowing}
%Input Data
\SetKwData{target}{$q_{goal}$}
%Variables
\SetKwData{minDistGoal}{$minDist2Goal$}
\SetKwData{total}{$totalPathLength$}
\SetKwData{pathToMin}{$length2lPoint$}
\SetKwData{traveled}{$pathTraveled$}
%leavePoint
\SetKwData{leavePoint}{$q_L^i$}
%localisation
\SetKwFunction{loc}{getRobotPosition()}
%compare euclidian distance between a point and the goal and the current position and the goal
%basic actions
\SetKwFunction{wall}{wallFollowing}

  \begin{algorithmic}
   %\Require{$dir$ is already specified}
    \Function{BoundaryFollowing}{$Boolean \ direction$}{\\
      \BlankLine
	  \While{\wall($direction$)}{
		updateData();
	  }
	  }
\EndFunction
   \end{algorithmic}
\end{algorithm}
\end{small}

\begin{tiny}
\begin{algorithm}%[H]
\label{AlgGen} \caption{Bug navigation Template Method}
\SetKwInOut{Input}{input}
\SetKwInOut{Output}{output}
%Input Data
\SetKwData{start}{$q_{start}$}
\SetKwData{target}{$q_{goal}$}
\SetKwData{distance}{$\varphi(p, \theta)$}
\SetKwData{mline}{$M-line$}
%Variables
\SetKwData{minDistGoal}{$minDist2Goal$}
\SetKwData{pathToMin}{$path2leavePoint$}
\SetKwData{total}{$totalPath$}
%hitPoint et leavePoint
\SetKwData{iterator}{$i$}
\SetKwData{hitPoint}{$q_H^i$}
\SetKwData{leavePoint}{$q_L^i$}
%List record
\SetKwData{hlist}{$H_{list}$}
\SetKwData{llist}{$L_{list}$}
\SetKwFunction{oldHit}{isEncounteredHitPoint}
\SetKwFunction{oldLeave}{isEncounteredLeavePoint}
%localisation
\SetKwData{position}{$x$}
%termination boolean
\SetKwData{termination}{termination}
%basic actions
\SetKwFunction{MotionToGoal}{motionToGoal()}
\SetKwFunction{BoundaryFollowing}{boundaryFollowing}
\SetKwFunction{wall}{wallFollowing}
\SetKwFunction{Stop}{stop()}
\SetKwFunction{GoTo}{goToPoint}
%Perception
\SetKwFunction{obstacleDetected}{obstacleInWay()}
\SetKwFunction{loc}{getRobotPosition()}
%Reachable goal?
\SetKwFunction{Reachable}{goalIsReachable}
\SetKwFunction{TReached}{goalReached}
%Euclidian distance
\SetKwFunction{euclid}{$d_e$}
%Specific to Alg1
\SetKwFunction{isMline}{isOnMline-V2}
%\SetKwFunction{closer}{closerToGoal-V2}
\SetKwFunction{rec}{setHitPoint}
\SetKwFunction{cpte}{discontinuityPointsTreatment}
\SetKwFunction{encountered}{encounteredPointsCondition}
\SetKwFunction{loopCond}{loopCondition}
\SetKwFunction{algo}{algorithmSpecificCondition}
\SetKwFunction{algoTr}{algoTreatment}
\SetKwFunction{loopTr}{loopTreatment}
\SetKwFunction{encounteredTr}{encounteredTreatment}
\SetKwFunction{tryToLeave}{tryToLeave}
\Input{Point \start, Point \target}
\Output{Boolean termination}
Init();
\termination $\gets$ false\;

	\While{\termination == false}{
	\If{\obstacleDetected == true} {
	\rec{\loc}\;
	{\cpte{}\;}

	\If{not \tryToLeave{\termination}}
			{\BoundaryFollowing(getDirection())\;}
    }
    \Else{\MotionToGoal;}
    }
\end{algorithm}
\end{tiny}
\subsubsection{Discussion}

The class diagram for 4 Bug algorithm classes is presented in figure \ref{BugTemplateMethod}.

Une sous-classe d'une algorithme pour chaque capteurs (IR, Laser par exemple)=> explosion résolu par délégation et éventuellement récursivement le pattern template method.

Bilan: Pour chaque algo de Bug, il faut écrire une classe.
On arrive à factoriser du code, on arrive mieux à voir les différences entre les algos.
Que faire si certains pts communs entre plusieurs algos ? => possible de factoriser dans des sous-classes.

TM ne capture pas bien les contraintes entre capteurs ou les conditions pour choisir tel algo ou bien un autre.

If we want to use this pattern to implement all Bug variants (20 versions ?), the hierarchy will then become very complicated to understand.

% In this example, we have shown only 4 variants of Bug. Nevertheless, Bug variants are about 20 (?) versions of algorithms. Implementing all \texttt{BugAlgorithm} subclasses become then very complicated to understand and too expensive to build all Bug family members.

In addition, it is error prone to not define constraints on subclasses and the data they must specify and use.(???)

Difficulté pour relire le code, car des opérations spécifiques sont implémentés dans la template method.

Template method should not be overwritten.
Problème de nommage ?


It is then much cheaper to build operations of the algorithm as components and to assemble desired family members from them.

This is our main motivation for using an alternate solution based on Software Product Lines (SPL).
SPL are easy to use, compact and generate only a configuration which interests the user.
In the next section, we present our software product line for Bug navigation family.
\begin{figure}[!htb]
\hspace{-1cm}
%\centering
\includegraphics[scale=0.35]{BugClassHierarchy.png}
\vspace{-2cm}
\caption{Bug Template method class hierarchy}
\label{BugTemplateMethod}
\end{figure}	


==> section32.tex <==

\subsection{Software Product Lines}
\subsubsection{Description}
Software Product Lines focus on capturing commonality and variability between several software products belonging to the same domain~\cite{Clements01}. Commonality gather assumptions that are true for all product members while variability concerns assumptions about how individual product members differ.
The SPL engineering process, as defined in the research literature~\cite{Clements01}, consists of two major steps: Domain Engineering and Application Engineering. 
The domain engineering step consists of designing a Feature Model (FM)~\cite{Kang90} to capture commonalities and variabilities within the SPL by means of features. We distinguish two main kinds of features: 1) \textit{Mandatory}: a mondatory feature is present in all product members of the SPL. 2) \textit{Optional}: an optional feature is only present in some members of the SPL. Features in the feature model can also be containers of other ones. In the \textit{OR containment}, at least one of the children features has to be present in a specific product. In contrast, in the \textit{Alternative} containment, one and only one of the children features can be chosen in a derived product. 
In addition to features, a feature model can also be defined with a set of constraints that specify dependencies between features.
In addition to the FM, the goal of the domain engineering step is to create a set of software assets (source code files, models..) that are necessary to implement the SPL. 
For each feature in the feature model, a set of assets is identified and implemented. \\
The Application Engineering step, also referred to as product derivation, consists of building product members of the SPL based on the result of domain engineering. Product derivation consists in :
\begin{itemize}
\item Instantiating the feature model and creating what is called \textit{configuration}.  A configuration is a combination of features which constitutes a specific product.
\item Customizing assets defined in the domain engineering step for the specific products.  
\end{itemize}


\subsubsection{Solution: A software product line for Bug family}
Our feature model for Bug navigation family \ref{FM} relies on the template method algorithm identified previously. The template method represents the central asset of the base feature which gathers commonalities among Bug algorithms.
Each operation invoked by the template method identified in the last section is represented as mandatory or optional feature and as concrete or abstract feature depending on its nature:
%\vspace{2cm}
\begin{figure*}[!htb]
\hspace{-1cm}
\includegraphics[scale=0.17]{./Figures/FMLastVersion.png} 
\caption{Feature model for Bug algorithms family}
\label{FM}
\end{figure*}

\begin{itemize}
\item Concrete operations are defined as concrete features.
\item Abstract operations are defined as abstract fe atures and their specializations are defined as concrete features. For example, in the figure \ref{FM}, \texttt{algorithm strategy} is defined as an abstract feature and the versions of specific-Leaving-Condition specialized in subclasses are defined as concrete features.
\item Hook operations are defined as concrete optional features. For instance, features \texttt{encounteredPoints}, \texttt{goalReachabilty} and \texttt{recordData} define respectively the operations \textit{encounteredPointsCondition()}, \textit{goalIsReachable()} and \textit{updateData()}. 
\item The feature Base represents the abstract class where the template method is defined. 
The template method, the inputs of the algorithm and declaration of hook operations (with an empty body by default) are defined in the feature Base.
\end{itemize}
\subsubsection{Limits of this approach}
Software product lines are designed to handle variabilites among softwares or/and applications. In our approach, we tried to identify an algorithmic software product line. Wa highlight several 
